Probing Acoustic Representations for Phonetic Properties

Pre-trained acoustic representations such as wav2vec and DeCoAR have attained impressive word error rates (WER) for speech recognition benchmarks, particularly when labeled data is limited. But little is known about what phonetic properties these various representations acquire, and how well they encode transferable features of speech. We compare features from two conventional and four pre-trained systems in some simple frame-level phonetic classification tasks, with classifiers trained on features from one version of the TIMIT dataset and tested on features from another. All contextualized representations offered some level of transferability across domains, and models pre-trained on more audio data give better results; but overall, DeCoAR, the system with the simplest architecture, performs best. This type of benchmarking analysis can thus uncover relative strengths of various proposed acoustic representations.

==> 09-candidate_figures.tex <==
\section{Candidate figures}
\begin{figure}[htb]
\begin{minipage}[b]{1\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/binary_class_distribution.pdf}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{Class distribution for binary tasks}
\end{figure}

\begin{figure*}[htb]
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/phone_class_distribution.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/phone_class_distribution_without_sil.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{Phone class distribution}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/mel_fbank.png}}
%  \vspace{2.0cm}
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/mfcc.png}}
%  \vspace{2.0cm}
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/wav2vec-large.png}}
%  \vspace{2.0cm}
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/vq-wav2vec.png}}
%  \vspace{2.0cm}
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/mockingjay.png}}
%  \vspace{2.0cm}
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/DeCoAR.png}}
%  \vspace{2.0cm}
\end{minipage}
\caption{Boxplots of overall performance (I also have similar boxplots for in-domain and cross-domain performance)}
\label{fig:overall_boxplots}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/majority.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/mel_fbank_no_context.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/mfcc_no_context.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{Similar to Figure \ref{fig:overall_boxplots}, Baseline performance}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=0.8\linewidth]{Candidate_figures/sad_combine_classifiers.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=0.8\linewidth]{Candidate_figures/syllable_combine_classifiers.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/sonorant_combine_classifiers.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/fricative_combine_classifiers.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.35\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/phone_combine_classifiers.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{Boxplots for each task. This is combining all the numbers. I also have similar boxplots for in-domain and cross-domain performance.}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_fricative_bad_rep.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_fricative_good_rep.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{A confusion matrix of fricative detection to compare the worst representation (Mockingjay, left) and the best representation (DeCoAR, right). Both are trained on FFMTIMIT and tested on FFMTIMIT, using SVM classifier.}
\label{fig:fricative_compare_rep}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_phone_bad_rep.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_phone_good_rep.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{Similar to Figure \ref{fig:fricative_compare_rep}, a confusion matrix of phoneme classification to compare the worst representation (Mockingjay, left) and the best representation (DeCoAR, right). Both are trained on TIMIT and tested on TIMIT, using LR classifier.}
\label{fig:phone_compare_rep}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.24\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_syllable.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.24\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_hardest_task.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.24\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_sonorant.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.24\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_easiest_task.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{Confusion matrices to compare binary prediction task difficulty. From left to right (syllable, fricative, sonorant, SAD): hardest task to easiest task based on conditional entropy.}
\label{fig:phone_compare_rep}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.45\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_fricative_mismatch.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.55\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_fricative_best.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{A confusion matrix of fricative detection to compare domain mismatch. Left: greatest mismatch, trained on TIMIT, tested on CTIMIT; Right: best domain adaptation, trained FFMTIMIT, tested on TIMIT. Both are using DeCoAR and NN classifier.}
\label{fig:fricative_mismatch}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_phone_bad_rep.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
  \centering
  \centerline{\includegraphics[width=1\linewidth]{Candidate_figures/cm_phone_good_rep.png}}
%  \vspace{2.0cm}
%   \centerline{(a)}\medskip
\end{minipage}
\caption{Similar to Figure \ref{fig:fricative_mismatch}, a confusion matrix of phoneme classification to compare domain mismatch. Left: the greatest mismatch, trained on TIMIT, tested on CTIMIT; Right: best domain adaptation, trained FFMTIMIT, tested on TIMIT. Both are using DeCoAR and LR classifier.}
\label{fig:phone_compare_rep}
\end{figure*}
